SAFE: Scalable Automatic Feature Engineering Framework for Industrial Tasks

Machine learning techniques have been widely applied in Internet companies for various tasks, acting as an essential driving force, and feature engineering has been generally recognized as a crucial tache when constructing machine learning systems. Recently, a growing effort has been made to the development of automatic feature engineering methods, so that the substantial and tedious manual effort can be liberated. However, for industrial tasks, the efficiency and scalability of these methods are still far from satisfactory. In this paper, we proposed a staged method named SAFE (Scalable Automatic Feature Engineering), which can provide excellent efficiency and scalability, along with requisite interpretability and promising performance. Extensive experiments are conducted and the results show that the proposed method can provide prominent efficiency and competitive effectiveness when comparing with other methods. What's more, the adequate scalability of the proposed method ensures it to be deployed in large scale industrial tasks.

==> Classification-Accuracies-3.tex <==
\begin{table*}[htbp]
\caption{Classification Accuracies-\uppercase\expandafter{\romannumeral3}}
\begin{center}
\begin{tabular}{|l|l|c|c|c|c|c|c|c|}
\hline
Dataset Name & Classifier & Origin & FCTree-A & FCTree-B & TFC & Random & Important & GSS\\
\hline
 & AdaBoost & 0.914838 & - & 0.917126 & 0.881657 & 0.917744 & 0.918343 & \textbf{0.920835}\\
 & Decision Tree & 0.879364 & 0.879682 & 0.880290 & 0.853235 & 0.882679 & 0.883106 & \textbf{0.887159}\\
 & Extremely Randomized Trees & 0.899812 & - & 0.908071 & 0.867411 & 0.910913 & 0.912128 & \textbf{0.919224}\\
 & \textit{k}-nearest neighbors & 0.812608 & - & 0.824981 & \textbf{0.855081} & 0.822195 & 0.823328 & 0.835035\\
mt-small & Logistic Regression & 0.858921 & - & 0.862718 & 0.761358 & 0.871637 & 0.872783 & \textbf{0.881912}\\
 & Multilayer Perceptron & 0.899803 & - & 0.906942 & 0.853909 & 0.908736 & 0.909613 & \textbf{0.917485}\\
 & Random Forest & 0.913617 & - & 0.913633 & 0.880662 & 0.916956 & 0.917542 & \textbf{0.919708}\\
 & Support Vector Machine & 0.868563 & - & 0.871728 & 0.772595 & 0.878620 & 0.880475 & \textbf{0.888269}\\
 & XGBoost & 0.977083 & - & 0.977453 & 0.961555 & 0.978384 & 0.978693 & \textbf{0.980239}\\
\hline
 & AdaBoost & 0.932245 & - & 0.936612 & 0.929998 & 0.939028 & 0.939690 & \textbf{0.940514}\\
 & Decision Tree & 0.919402 & 0.915665 & 0.921934 & 0.906690 & 0.921166 & 0.921497 & \textbf{0.925997}\\
 & Extremely Randomized Trees & 0.941345 & - & 0.943469 & 0.942558 & 0.945582 & 0.943706 & \textbf{0.949360}\\
 & \textit{k}-nearest neighbors & 0.891170 & - & 0.893382 & \textbf{0.917105} & 0.895794 & 0.897316 & 0.902947\\
fanqizha-small & Logistic Regression & 0.894698 & - & 0.897744 & 0.894692 & 0.903809 & 0.904008 & \textbf{0.910687}\\
 & Multilayer Perceptron & 0.931346 & - & 0.938858 & 0.927191 & 0.937796 & 0.936259 & \textbf{0.942569}\\
 & Random Forest & 0.946867 & - & 0.945674 & 0.938805 & 0.947730 & 0.947487 & \textbf{0.950252}\\
 & Support Vector Machine & 0.899678 & - & 0.902052 & 0.896976 & 0.908438 & 0.908168 & \textbf{0.915502}\\
 & XGBoost & 0.986930 & - & 0.987128 & 0.983496 & 0.987390 & 0.987993 & \textbf{0.988608}\\
\hline
 & AdaBoost & 0.743066 & - & 0.744527 & 0.722400 & 0.747787 & 0.747654 & \textbf{0.754792}\\
 & Decision Tree & 0.682101 & 0.678077 & 0.681664 & 0.662477 & 0.682372 & 0.685779 & \textbf{0.687918}\\
 & Extremely Randomized Trees & 0.709567 & - & 0.719583 & 0.669446 & 0.724839 & 0.726319 & \textbf{0.732630}\\
 & \textit{k}-nearest neighbors & 0.665213 & - & 0.667057 & \textbf{0.679392} & 0.669649 & 0.669855 & 0.673014\\
fraud-small & Logistic Regression & 0.688210 & - & 0.689558 & 0.501339 & 0.697231 & \textbf{0.698186} & 0.696779\\
 & Multilayer Perceptron & 0.746817 & - & 0.750719 & 0.668890 & 0.752260 & 0.752416 & \textbf{0.754704}\\
 & Random Forest & 0.730843 & - & 0.732451 & 0.701871 & 0.741696 & 0.742084 & \textbf{0.744792}\\
 & Support Vector Machine & 0.692445 & - & 0.694835 & 0.503153 & 0.702871 & \textbf{0.703689} & 0.702000\\
 & XGBoost & 0.849624 & - & 0.850926 & 0.816105 & 0.849442 & 0.851075 & \textbf{0.854993}\\
\hline
 & AdaBoost & 0.828556 & - & 0.829675 & 0.819700 & 0.830280 & 0.829678 & \textbf{0.831328}\\
 & Decision Tree & 0.760904 & 0.758109 & 0.759383 & 0.755522 & 0.760582 & 0.761017 & \textbf{0.762435}\\
 & Extremely Randomized Trees & 0.812881 & - & 0.808249 & 0.801073 & 0.813519 & 0.815395 & \textbf{0.816377}\\
 & \textit{k}-nearest neighbors & 0.800689 & - & 0.800647 & 0.792191 & 0.801069 & 0.802318 & \textbf{0.803814}\\
huabei-small & Logistic Regression & 0.825652 & - & 0.826568 & 0.817733 & 0.827250 & 0.827660 & \textbf{0.827664}\\
 & Multilayer Perceptron & 0.834766 & - & 0.835636 & 0.822371 & \textbf{0.835703} & 0.835137 & 0.835271\\
 & Random Forest & 0.816010 & - & 0.812885 & 0.805603 & 0.817565 & 0.817149 & \textbf{0.818357}\\
 & Support Vector Machine & 0.826790 & - & 0.827206 & 0.820980 & 0.827675 & 0.828223 & \textbf{0.828625}\\
 & XGBoost & 0.912543 & - & 0.912079 & 0.904342 & 0.913149 & 0.913195 & \textbf{0.914277}\\
\hline
 & AdaBoost & 0.821960 & - & 0.823815 & 0.823389 & 0.824676 & 0.822361 & \textbf{0.826262}\\
 & Decision Tree & 0.749226 & 0.744776 & 0.751070 & 0.750506 & 0.751095 & 0.749056 & \textbf{0.754021}\\
 & Extremely Randomized Trees & 0.800758 & - & 0.806522 & 0.808938 & 0.808167 & 0.807972 & \textbf{0.811816}\\
 & \textit{k}-nearest neighbors & 0.770836 & - & 0.785201 & \textbf{0.790861} & 0.774277 & 0.778266 & 0.786266\\
weidai-small & Logistic Regression & 0.817435 & - & 0.821555 & 0.818483 & 0.820685 & 0.820131 & \textbf{0.823834}\\
 & Multilayer Perceptron & 0.825046 & - & 0.827022 & \textbf{0.829359} & 0.825380 & 0.826227 & 0.827683\\
 & Random Forest & 0.804841 & - & 0.809030 & 0.810404 & 0.809521 & 0.810187 & \textbf{0.812389}\\
 & Support Vector Machine & 0.817860 & - & 0.821175 & 0.817904 & 0.821428 & 0.820328 & \textbf{0.823921}\\
 & XGBoost & 0.905784 & - & 0.906674 & 0.906282 & 0.907754 & 0.906790 & \textbf{0.908860}\\
\hline
\end{tabular}
\label{Classification Accuracies 3}
\end{center}
\end{table*}


==> Classification-Performance-Benchmark.tex <==
\begin{table*}[htbp]
\label{Classification performance on benchmark data sets}
\caption{Classification performance on benchmark data sets}
\begin{center}
\scalebox{0.95}{
\begin{tabular}{cccccccc|cccccccc}
\hline
Dataset & CLF & ORIG & FCT & TFC & RAND & IMP & SAFE & Dataset & CLF & ORIG & FCT & TFC & RAND & IMP & SAFE\\
\hline
 & AB & 52.10 & 78.27 & 87.33 & 88.20 & 88.30 & \textbf{88.92} & & AB & 99.55 & 99.38 & 96.59 & \textbf{99.62} & 99.58 & 99.53\\
 & DT & 54.38 & 70.78 & 77.37 & 77.37 & 77.43 & \textbf{78.32} & & DT & 98.20 & 98.90 & 96.38 & 98.83 & 98.78 & \textbf{98.99}\\
 & ET & 55.54 & 76.64 & \textbf{88.44} & 85.77 & 86.03 & 88.33 & & ET & 99.83 & 99.76 & 96.95 & 99.88 & 99.88 & \textbf{99.93}\\
 & \textit{k}NN & 51.84 & 78.69 & \textbf{94.81} & 93.01 & 92.69 & 93.66 & & \textit{k}NN & 99.86 & 99.75 & 97.45 & 99.88 & 99.90 & \textbf{99.96}\\
valley & LR & 58.54 & 80.69 & 92.53 & 93.31 & 93.39 & \textbf{93.80} & banknote & LR & 94.80 & 96.47 & 88.14 & 97.24 & 97.12 & \textbf{97.79}\\
 & MLP & 59.63 & 81.27 & 92.71 & 93.93 & 93.97 & \textbf{94.08} & & MLP & 98.77 & 98.51 & 88.07 & 99.25 & 99.21 & \textbf{99.36}\\
 & RF & 54.54 & 76.31 & 87.06 & 84.34 & 84.34 & \textbf{87.11} & & RF & 99.01 & 99.46 & 96.98 & 99.51 & 99.48 & \textbf{99.57}\\
 & SVM & 65.62 & 81.53 & 93.39 & 94.22 & 94.38 & \textbf{94.94} & & SVM & 98.29 & 98.03 & 88.22 & 98.56 & 98.53 & \textbf{98.64}\\
 & XGB & 54.75 & 86.92 & 94.75 & 95.14 & 95.23 & \textbf{95.68} & & XGB & 99.83 & 99.88 & 99.25 & 99.91 & 99.89 & \textbf{99.91}\\
\hline
 & AB & 85.15 & 85.24 & 86.22 & 85.60 & 87.54 & \textbf{90.19} & & AB & 93.61 & 93.49 & 92.06 & 93.61 & 93.59 & \textbf{93.74}\\
 & DT & 85.50 & 85.75 & 84.01 & 85.69 & 86.11 & \textbf{87.53} & & DT & 91.28 & 91.06 & 90.72 & 91.51 & 91.65 & \textbf{92.18}\\
 & ET & 91.65 & 91.31 & 88.44 & 91.59 & 92.27 & \textbf{92.79} & & ET & 94.22 & 93.09 & 92.43 & 94.34 & \textbf{94.48} & 94.45\\
 & \textit{k}NN & 83.95 & \textbf{91.98} & 88.46 & 85.03 & 88.03 & 89.08 & & \textit{k}NN & 89.10 & 89.30 & \textbf{91.21} & 90.38 & 90.44 & 91.09\\
gina & LR & 85.12 & 86.23 & 86.38 & 85.61 & 87.34 & \textbf{90.35} & spambase & LR & 87.71 & 87.86 & 83.68 & 89.48 & 89.53 & \textbf{90.15}\\
 & MLP & 93.09 & 93.81 & 89.09 & 93.21 & 93.75 & \textbf{93.83} & & MLP & 93.81 & 93.43 & 91.04 & 93.84 & 93.81 & \textbf{93.94}\\
 & RF & 90.50 & 90.45 & 87.96 & 90.40 & 91.23 & \textbf{91.86} & & RF & 93.94 & 92.74 & 92.58 & 93.96 & 94.01 & \textbf{94.17}\\
 & SVM & 81.40 & 86.25 & 84.90 & 82.07 & 84.58 & \textbf{88.59} & & SVM & 90.21 & 90.08 & 86.51 & 91.13 & 91.07 & \textbf{91.60}\\
 & XGB & 97.76 & 97.33 & 96.46 & 97.74 & 97.71 & \textbf{97.90} & & XGB & 98.27 & 98.18 & 97.86 & 98.34 & 98.41 & \textbf{98.46}\\
\hline
 & AB & 76.90 & 79.25 & 73.98 & 79.70 & 79.64 & \textbf{79.90} & & AB & \textbf{85.62} & 85.43 & 83.84 & 85.47 & 85.40 & 85.44\\
 & DT & \textbf{84.07} & 83.92 & 79.68 & 83.65 & 83.95 & 84.05 & & DT & 79.76 & 79.63 & 78.41 & 79.99 & 80.12 & \textbf{80.13}\\
 & ET & 86.31 & 85.69 & 82.07 & 87.03 & 86.87 & \textbf{87.09} & & ET & 84.41 & 84.49 & 82.92 & 85.03 & 84.90 & \textbf{85.06}\\
 & \textit{k}NN & 83.92 & 83.65 & 79.59 & 84.60 & 84.47 & \textbf{84.65} & & \textit{k}NN & 83.91 & \textbf{84.91} & 83.49 & 84.56 & 84.59 & 84.80\\
phoneme & LR & 66.32 & 66.91 & 64.69 & 67.21 & 67.42 & \textbf{67.47} & wind & LR & 85.12 & 85.18 & 83.90 & 85.28 & 85.28 & \textbf{85.34}\\
 & MLP & 76.56 & 77.23 & 72.94 & 78.25 & 78.27 & \textbf{78.39} & & MLP & \textbf{86.77} & 86.52 & 84.93 & 86.67 & 86.66 & 86.66\\
 & RF & 85.72 & 85.72 & 81.25 & 86.02 & 86.13 & \textbf{86.14} & & RF & 84.66 & 84.65 & 83.39 & 85.10 & 85.11 & \textbf{85.24}\\
 & SVM & 66.88 & 67.21 & 65.20 & 68.15 & 68.47 & \textbf{68.68} & & SVM & 85.09 & 85.12 & 84.24 & 85.32 & 85.30 & \textbf{85.46}\\
 & XGB & \textbf{93.81} & 93.56 & 90.96 & 93.63 & 93.67 & 93.58 & & XGB & 93.72 & 93.71 & 92.51 & 93.69 & \textbf{93.74} & 93.70\\
\hline
 & AB & 87.16 & \textbf{87.16} & 81.58 & 87.08 & 87.07 & 87.14 & & AB & 73.48 & 74.61 & 73.48 & 74.76 & 74.59 & \textbf{75.18}\\
 & DT & 82.92 & \textbf{83.46} & 78.38 & 83.28 & 83.37 & 83.46 & & DT & 82.37 & 83.46 & 82.55 & 83.76 & 83.55 & \textbf{83.99}\\
 & ET & 83.32 & 84.14 & 79.04 & 85.04 & 85.64 & \textbf{86.25} & & ET & 89.24 & 90.34 & 89.41 & 90.31 & 90.27 & \textbf{90.67}\\
 & \textit{k}NN & 85.72 & 85.51 & 78.95 & 86.08 & 86.41 & \textbf{86.60} & & \textit{k}NN & 86.32 & 89.38 & 86.49 & 89.37 & 89.48 & \textbf{90.34}\\
ailerons & LR & 87.47 & 87.55 & 80.61 & 87.58 & 87.60 & \textbf{87.64} & eeg-eye & LR & 51.25 & 52.92 & 50.61 & 53.69 & 53.73 & \textbf{53.75}\\
 & MLP & 87.54 & 87.79 & 80.09 & 87.83 & \textbf{87.99} & 87.96 & & MLP & 54.58 & 55.71 & 52.52 & 55.85 & 55.81 & \textbf{56.64}\\
 & RF & 84.46 & 85.60 & 79.29 & 86.05 & 86.39 & \textbf{86.82} & & RF & 88.21 & 89.02 & 87.84 & 89.03 & 88.99 & \textbf{89.34}\\
 & SVM & 87.49 & 87.55 & 80.54 & 87.65 & 87.66 & \textbf{87.75} & & SVM & 54.56 & 56.56 & 54.62 & 56.97 & 56.80 & \textbf{57.23}\\
 & XGB & 95.48 & 95.62 & 90.62 & 95.58 & 95.60 & \textbf{95.64} & & XGB & 91.70 & 93.02 & 91.63 & 92.89 & 92.84 & \textbf{93.28}\\
\hline
 & AB & 81.01 & 81.89 & 77.72 & 82.53 & 82.53 & \textbf{82.95} & & AB & 93.13 & 93.47 & 92.46 & 93.66 & 93.73 & \textbf{94.04}\\
 & DT & 79.89 & 80.04 & 77.51 & 80.45 & 80.43 & \textbf{80.67} & & DT & 93.26 & 92.90 & 91.95 & 93.06 & 93.14 & \textbf{93.28}\\
 & ET & 82.64 & 81.60 & 80.48 & 83.29 & 83.41 & \textbf{83.76} & & ET & 95.58 & 95.44 & 95.07 & 95.56 & 95.63 & \textbf{95.69}\\
 & \textit{k}NN & 79.55 & 80.17 & 79.40 & 80.70 & 80.89 & \textbf{81.10} & & \textit{k}NN & 94.25 & 94.09 & 93.29 & 94.29 & 94.32 & \textbf{94.44}\\
magic & LR & 74.24 & 75.84 & 75.84 & 77.00 & 76.92 & \textbf{77.31} & nomao & LR & 93.30 & 93.12 & 91.93 & 93.73 & 93.74 & \textbf{93.76}\\
 & MLP & 83.66 & 83.70 & 80.38 & 84.26 & 84.28 & \textbf{84.43} & & MLP & 95.00 & 94.84 & 91.94 & 94.98 & 95.02 & \textbf{95.19}\\
 & RF & 83.70 & 82.93 & 80.87 & 84.15 & 84.21 & \textbf{84.43} & & RF & 95.53 & 95.33 & 94.27 & 95.49 & 95.52 & \textbf{95.62}\\
 & SVM & 74.09 & 75.92 & 75.34 & 76.94 & 76.89 & \textbf{77.14} & & SVM & 93.54 & 93.42 & 92.01 & 94.01 & 94.03 & \textbf{94.05}\\
 & XGB & 92.14 & 92.21 & 89.74 & 92.68 & 92.70 & \textbf{92.88} & & XGB & 98.95 & 98.97 & 98.73 & 99.01 & 99.05 & \textbf{99.13}\\
\hline
 & AB & 67.05 & 67.83 & 67.09 & 67.37 & 67.46 & \textbf{68.95} & & AB & 85.81 & 85.86 & 83.88 & 86.52 & 86.48 & \textbf{86.69}\\
 & DT & 70.88 & 70.67 & 68.28 & 70.24 & 70.15 & \textbf{70.94} & & DT & 78.44 & 78.42 & 75.81 & \textbf{79.53} & 79.21 & 79.27\\
 & ET & 64.65 & 67.40 & 65.39 & 68.09 & 68.70 & \textbf{68.77} & & ET & 85.53 & 85.17 & 83.03 & 85.90 & 85.89 & \textbf{86.19}\\
 & \textit{k}NN & 61.49 & 64.75 & \textbf{68.20} & 62.97 & 63.57 & 64.76 & & \textit{k}NN & 78.58 & 81.64 & \textbf{82.19} & 79.24 & 79.97 & 81.88\\
bank & LR & 65.03 & 65.98 & 61.16 & 66.03 & 66.03 & \textbf{66.28} & vehicle & LR & 85.66 & 85.68 & 83.02 & 85.74 & 85.71 & \textbf{85.96}\\
 & MLP & 72.37 & 72.36 & 68.26 & 71.79 & \textbf{72.70} & 72.26 & & MLP & 86.79 & \textbf{87.10} & 83.27 & 86.63 & 86.48 & 87.03\\
 & RF & 66.54 & 66.29 & 65.51 & 67.53 & 67.71 & \textbf{68.24} & & RF & 85.55 & 85.18 & 82.93 & 86.28 & 86.16 & \textbf{86.50}\\
 & SVM & 63.95 & 64.13 & 60.61 & 64.15 & 64.28 & \textbf{64.44} & & SVM & 85.31 & 85.33 & 82.54 & 85.48 & 85.37 & \textbf{85.81}\\
 & XGB & 91.84 & 91.98 & 90.77 & 91.90 & 92.07 & \textbf{92.29} & & XGB & 91.86 & 92.05 & 90.85 & 92.30 & 92.29 & \textbf{92.47}\\
\hline
\end{tabular}
}
\end{center}
\end{table*}


==> Classification-Performance-Business.tex <==
\begin{table}[htbp]
\label{Classification performance of business data sets}
\caption{Classification performance of business data sets}
\begin{center}
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{cccccc}
\hline
Dataset & CLF & ORIG & RAND & IMP & SAFE\\
\hline
 & LR & 89.64 & 89.77 & 89.72 & \textbf{89.86}\\
Data1 & RF & 86.98 & 88.16 & 88.45 & \textbf{89.20}\\
 & XGB & 89.77 & 89.96 & 90.07 & \textbf{90.33}\\
\hline
 & LR & 89.64 & 89.77 & 89.72 & \textbf{89.86}\\
Data2 & RF & 86.98 & 88.16 & 88.45 & \textbf{89.20}\\
& XGB & 89.77 & 89.96 & 90.07 & \textbf{90.33}\\
\hline
\end{tabular}
}
\end{center}
\end{table}


==> Data-Sets-Bussiness.tex <==
\begin{table}[htbp]
	\label{The information of the bussiness data sets}
	\caption{The information of the bussiness data sets}
	\begin{center}
		\begin{tabular}{lcccc}
			\hline
			Dataset & \#Train & \#Valid & \#Test & \#Dim \\
			\hline
			Data1 & 1  &  1&  1& 1 \\
			Data2 & 1 &  1& 1 & 1\\
			\hline
		\end{tabular}
		
	\end{center}
\end{table}

==> Data-Sets-Public.tex <==
\begin{table}[htbp]
\caption{The information of the benchmark data sets}
\begin{center}
\setlength{\tabcolsep}{4mm}{
\begin{tabular}{lcccc}
\hline
Dataset & \#Train & \#Valid & \#Test & \#Dim\\
\hline
valley & 900 & - & 312 & 100\\
banknote & 1,000 & - & 372 & 4\\
gina & 2,800 & - & 668 & 970\\
spambase & 3,800 & - & 801 & 57\\
phoneme & 4,500 & - & 904 & 5\\
wind & 5,000 & - & 1,574 & 14\\
ailerons & 9,000 & 2,000 & 2,750 & 40\\
eeg-eye & 10,000 & 2,000 & 2,980 & 14\\
magic & 13,000 & 3,000 & 3,020 & 10\\
nomao & 22,000 & 6,000 & 6,000 & 118\\
bank & 35,211 & 4,000 & 6,000 & 51\\
vehicle & 60,000 & 18,528 & 20,000 & 100\\
\hline
\end{tabular}
}
\label{The information of the public data sets}
\end{center}
\end{table}

==> Executing-Time.tex <==
\begin{table}[htbp]
\caption{Execution time (in second)}
\begin{center}
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{lccccc}
\hline
Dataset & FCT & TFC & RAND & IMP & SAFE\\
\hline
valley & 9.80 & 228.93 & 0.55 & 0.65 & 0.73\\
banknote & 0.16 & 0.27 & 0.08 & 0.31 & 0.12\\
gina & 84.03 & 95.73 & 3.39 & 5.28 & 5.31\\
spambase & 23.84 & 262.11 & 2.85 & 3.23 & 3.17\\
phoneme & 10.83 & 2.48 & 0.46 & 0.58 & 0.51\\
wind & 25.03 & 22.87 & 2.13 & 2.39 & 2.33\\
ailerons & 80.73 & 336.53 & 2.12 & 2.57 & 2.72\\
egg-eye & 58.88 & 42.13 & 1.09 & 1.20 & 1.18\\
magic & 52.45 & 36.79 & 2.55 & 2.96 & 3.32\\
nomao & 104.59 & 1469.19 & 22.22 & 26.61 & 28.82\\
bank & 838.17 & 552.48 & 13.70 & 13.81 & 12.28\\
vehicle & 1355.19 & 2748.89 & 52.86 & 40.34 & 62.14\\
\hline
\end{tabular}
}
\label{Executing time}
\end{center}
\end{table}


==> Feature-Importance.tex <==
\begin{figure*}[htbp]
\centering
\subfigure[valley]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/valley.png}
    \end{minipage}
}%
\subfigure[banknote]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/banknote.png}
    \end{minipage}
}%
\subfigure[gina]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/gina.png}
    \end{minipage}
}%

\subfigure[spambase]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/spambase.png}
    \end{minipage}
}%
\subfigure[phoneme]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/phoneme.png}
    \end{minipage}
}%
\subfigure[wind]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/wind.png}
    \end{minipage}
}%

\subfigure[ailerons]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/ailerons.png}
    \end{minipage}
}%
\subfigure[eeg-eye]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/eeg-eye.png}
    \end{minipage}
}%
\subfigure[magic]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/magic.png}
    \end{minipage}
}%

\subfigure[nomao]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/nomao.png}
    \end{minipage}
}%
\subfigure[bank]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/bank.png}
    \end{minipage}
}%
\subfigure[vehicle]{
    \begin{minipage}[t]{0.32\linewidth}
    %\centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Feature-Importance/vehicle.png}
    \end{minipage}
}%
\caption{Feature importance}
\label{Feature importance}
\end{figure*}

==> Feature-Stability.tex <==
\begin{table}[htbp]
\caption{Feature stability}
\begin{center}
\setlength{\tabcolsep}{4mm}{
\begin{tabular}{lcccc}
\hline
Dataset & FCT & RAND & IMP & SAFE\\
\hline
valley & 0.6991 & 0.4933 & 0.4947 & \textbf{0.4710}\\
banknote & 0.4405 & 0.3233 & 0.3174 & \textbf{0.1197}\\
gina & 0.5700 & 0.4639 & 0.4739 & \textbf{0.4163}\\
spambase & 0.5101 & 0.4571 & 0.4399 & \textbf{0.3587}\\
phoneme & \textbf{0.1947} & 0.3269 & 0.3294 & 0.2616\\
wind & 0.3707 & 0.3608 & 0.3570 & \textbf{0.3230}\\
ailerons & 0.4440 & 0.4590 & 0.3963 & \textbf{0.3330}\\
egg-eye & 0.3529 & 0.3768 & 0.3741 & \textbf{0.3212}\\
magic & \textbf{0.1847} & 0.3306 & 0.3384 & 0.2620\\
nomao & 0.5061 & 0.5032 & 0.4735 & \textbf{0.4065}\\
bank & 0.3713 & 0.4240 & 0.4072 & \textbf{0.2853}\\
\hline
\end{tabular}
}
\label{Feature stability}
\end{center}
\end{table}


==> Information-Value.tex <==
\begin{table}[htbp]
\caption{Information Value}
\begin{center}
\setlength{\tabcolsep}{6mm}{
\begin{tabular}{c|c}
\hline
Information Value & Predictive Power\\
\hline
$0$ to $0.02$ & Useless for prediction\\
$0.02$ to $0.1$ & Weak predictor\\
$0.1$ to $0.3$ & Medium predictor\\
$0.3$ to $0.5$ & Strong predictor\\
$>0.5$ & Extremely strong predictor\\
\hline
\end{tabular}
}
\label{Information Value}
\end{center}
\end{table}

==> Iteration.tex <==
\begin{figure*}[htbp]
\centering
\subfigure[valley]{
    \begin{minipage}[t]{0.325\linewidth}
    \centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Iteration/valley.png}
    \end{minipage}%
}%
\subfigure[banknote]{
    \begin{minipage}[t]{0.325\linewidth}
    \centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Iteration/banknote.png}
    \end{minipage}%
}%
\subfigure[gina]{
    \begin{minipage}[t]{0.325\linewidth}
    \centering
    \includegraphics[width=2.2in,trim={0.9cm 0cm 2.0cm 1.1cm},clip]{ICDE2020/fig/Iteration/gina.png}
    \end{minipage}%
}%
\centering
\caption{Performance at different iterations}
\label{Performance at different iterations}
\end{figure*}

==> Pearson.tex <==
\begin{table}[htbp]
\caption{Pearson Correlation}
\begin{center}
\setlength{\tabcolsep}{4mm}{
\begin{tabular}{c|c}
\hline
Pearson Correlation Coefficient & Correlation\\
\hline
$0$ to $0.2$ & Very weak or no correlation\\
$0.2$ to $0.4$ & Weak correlation\\
$0.4$ to $0.6$ & Moderate correlation\\
$0.6$ to $0.8$ & Strong correlation\\
$0.8$ to $1$ & Extremely strong correlation\\
\hline
\end{tabular}
}
\label{Pearson Correlation Coefficient}
\end{center}
\end{table}
